Thoughtful Adoption of NLP for Civic Participation: Understanding Differences Among Policymakers

Natural language processing (NLP) tools have the potential to boost civic participation and enhance democratic processes because they can significantly increase governments' capacity to gather and analyze citizen opinions. However, their adoption in government remains limited, and harnessing their benefits while preventing unintended consequences remains a challenge. While prior work has focused on improving NLP performance, this work examines how different internal government stakeholders influence NLP tools' thoughtful adoption. We interviewed seven politicians (politically appointed officials as heads of government institutions) and thirteen public servants (career government employees who design and administrate policy interventions), inquiring how they choose whether and how to use NLP tools to support civic participation processes. The interviews suggest that policymakers across both groups focused on their needs for career advancement and the need to showcase the legitimacy and fairness of their work when considering NLP tool adoption and use. Because these needs vary between politicians and public servants, their preferred NLP features and tool designs also differ. Interestingly, despite their differing needs and opinions, neither group clearly identifies who should advocate for NLP adoption to enhance civic participation or address the unintended consequences of a poorly considered adoption. This lack of clarity in responsibility might have caused the governments' low adoption of NLP tools. We discuss how these findings reveal new insights for future HCI research. They inform the design of NLP tools for increasing civic participation efficiency and capacity, the design of other tools and methods that ensure thoughtful adoption of AI tools in government, and the design of NLP tools for collaborative use among users with different incentives and needs.

==> Tables/interview.tex <==
\begin{table*}[h!]
    \centering
    \caption{Interview structure}
    \begin{tabular}{|m{0.2\textwidth}|m{0.69\textwidth}|}
    \toprule
       {\cellcolor{lightgray!50!}\textbf{Interview phase}} & {\cellcolor{lightgray!50!}\textbf{Description}} \\
       \hline
       1) Participation processes & We asked participants to describe a participatory process in which they have been involved. We probed to get details about participant roles, involvement, challenges, and challenges encountered.\\
       \midrule
       2a) Critical analysis of using NLP in participation processes & We asked participants to describe a process in which they had used NLP tools. In particular, we probed about the tool's role(s) and perceived advantages,  challenges, and whether it changed how they worked with stakeholders and the outputs of the process.\\
       \midrule
       2b) Speculation in using AI in participation processes & We asked participants to think about the process they described and speculate how it could change using NLP tools. In particular, we probed about the tool's role(s) and potential advantages, challenges, and whether it would change how they work with stakeholders and the outputs of the process.\\
       \midrule
       3) Risks and guardrails & We asked participants to describe the main risks and challenges they believe exist in using NLP for participation processes. If not mentioned, we probed about their thoughts on accountability, transparency, explanations, privacy, automation, changes in work practice, etc. We then asked how they think the use of these tools could harm constituents and what elements should be in place to prevent that from happening. Finally, we probed about how they would address risks, challenges, and potential tensions with usability.\\
       
       \bottomrule
    \end{tabular}
    \label{tab:interviews}
\end{table*}
